Real-World Textured Things: a Repository of Textured Models Generated with Modern Photo-Reconstruction Tools

We are witnessing a proliferation of textured 3D models captured from the real world with automatic photo-reconstruction tools. Digital 3D models of this class come with a unique set of characteristics and defects -- especially concerning their parametrization -- setting them starkly apart from 3D models originating from other, more traditional, sources. We study this class of 3D models by collecting a significant number of representatives and quantitatively evaluating their quality according to several metrics. These include a new invariant metric we design to assess the fragmentation of the UV map, one of the main weaknesses hindering the usability of these models. Our results back the widely shared notion that such models are not fit for direct use in downstream applications (such as videogames), and require challenging processing steps. Regrettably, existing automatic geometry processing tools are not always up to the task: for example, we verify that available tools for UV optimization often fail due mesh inconsistencies, geometric and topological noise, excessive resolution, or other factors; moreover, even when an output is produced, it is rarely a significant improvement over the input (according to the aforementioned measures). Therefore, we argue that further advancements are required specifically targeted at this class of models. Towards this goal, we share the models we collected in the form of a new public repository, Real-World Textured Things (RWTT), a benchmark to systematic field-test and compare algorithms. RWTT consists of 568 carefully selected textured 3D models representative of all the main modern off-the-shelf photo-reconstruction tools. The repository is available at http://texturedmesh.isti.cnr.it/ and is browsable by metadata collected during experiments, and comes with a tool, TexMetro, providing the same set of measures for generic UV mapped datasets.

==> dataset.tex <==
\section{Dataset curation and organization}\label{sec:organization}

As mentioned in the introduction, one of the motivations behind the creation of \dataset{} is to provide researchers and developers a challenging testbed of textured 3D models indicative of the actual models that can be encountered in practice.
Rather than creating the models in-house, we have collected publicly available models created and released by professionals practitioners and hobbyists.
This strategy has been successfully employed by other authors (e.g. \cite{thingi, abc}) and has the important advantage of allowing us to include models generated with various software packages, which is crucial to obtain a representative sample of the 3D data that can be found in the real world.
In particular, it is reasonable to expect the emergence of some common traits characterizing the geometry and textures of the models in the dataset according to the implementation details and algorithmic choices of different reconstruction pipelines.

At the time of writing, the dataset features 561 models collected from two sources: SketchFab \citep{sketchfab} and the Smithsonian 3D Program \citep{smithsonian}.
SketchFab is a popular online repository for publishing and sharing 3D content, used by thousands of users and constantly growing.
It features a large collection of 3D models reconstructed from photographs, and conveniently exposes a web API to collect automatically retrieve metadata such as the model author, description and tags among others.
The Smithsonian 3D Program is a digitization project from the Smithsonian Institution which published and made available a selection of 3D reconstructions of artifacts and relics.

We plan to keep the dataset updated by adding new models in the future.

The dataset is organized as a collection of folders using a progressive naming scheme to facilitate automatic processing of the 3D models.
Each model in the dataset is assigned a progressive identifier $ID$ and is stored in a folder named RWT$ID$.

For each model, we provide the following data:
\begin{itemize}
\item The 3D model in OBJ format and its material file
\item The textures referenced by the material file
\item A JSON file with the provenance metadata of the model
\item A JSON file with geometric and parametrization measures 
\end{itemize}

Although the original models and textures came in a variety of formats, we have converted all of them to unique formats for convenience.
All the models are provided as .OBJ files, and the textures as .PNG images.
Whenever necessary, the conversion only involved the file formats while the 3D and image data was left untouched; the models archived in their original formats are available separately.
The textures we provide mostly encode just surface colors; however, many original archives also contain textures storing other signals such as surface normals, specularity and ambient occlusion.

Each model comes with its \emph{metadata.json} file reporting information such as the name of the 3D model, the author, the license under which the model was released, a textual description of the model provided by the author, the date in which the model was published, a collection of tags chosen by the author, and a resource identifier.
For models obtained from SketchFab the resource identifier is the URI assigned from SketchFab itself, whereas for the ones obtained from the Smithsonian 3D Program the URI is the link to the web-page showcasing the model.
When available, we also include the software used to generate the model and a semantic category we assigned to the models for classification purposes.

Overall, the dataset includes 561 models created by 128 unique authors using at least 18 different acquisition pipelines; the models were published across a 6 year time span from 2013 to 2019.

We have been careful to almost exclusively include models that have been released with permissive licenses so as to allow anyone using the dataset to freely share their results: all of the models from SketchFab are released under various declinations of the Creative Commons 4.0 license; the models from the Smithsonian 3D Project follow the ``Smithsonian Terms of Use'', allowing fair use as long as the original source is cited.



Finally, we also include a \emph{texmetro.json} file generated with the \texmetro{} tool.
This JSON file contains information about the geometry, parameterization and textures of the models; a detailed description of the \texmetro{} tool and its output is given in section \ref{sec:texmetro}.





==> pre.tex <==


\newcommand{\dataset}{Real-World Textured Things}
\newcommand{\ds}{RWTT}
\newcommand{\texmetro}{TexMetro}

\newcommand{\andrea}[1]{\textbf{[Andrea]\textcolor{red}{#1}}}
\newcommand{\paolo}[1]{\textbf{[Paolo]\textcolor{green}{#1}}}
\newcommand{\marco}[1]{\textbf{[Marco]\textcolor{blue}{#1}}}






